A Critical Look at Smart Wheelchairs

Research into smart wheelchairs has been conducted for decades, but we have yet to see the widespread use of this technology among full-time wheelchair users. We argue that the main reason for this is that there is a mismatch between research and the actualities of using a powered mobility device in the real world. Based on our own research experiences, we enumerate some of these disparities, and offer some suggestions for where work in smart wheelchairs might focus in the coming years.

==> acknowledgements.tex <==
\section*{ACKNOWLEDGMENTS}

The authors would like to thank the ALS Association of Oregon and SW Washington, and especially Mary Rebar, for their support and for the loan of wheelchair hardware.  David Knight supplied invaluable technical advice on our powered wheelchairs.  We would especially like to thank Eric Valor, Steve Saling, and Henry Evans for their input, feedback, and insight into what it means to depend on a mobility device, powered or otherwise.
